Byzantine-Robust Learning on Heterogeneous Data via Gradient Splitting

Federated learning has exhibited vulnerabilities to Byzantine attacks, where the Byzantine attackers can send arbitrary gradients to a central server to destroy the convergence and performance of the global model. A wealth of robust AGgregation Rules (AGRs) have been proposed to defend against Byzantine attacks. However, Byzantine clients can still circumvent robust AGRs when data is non-Identically and Independently Distributed (non-IID). In this paper, we first reveal the root causes of performance degradation of current robust AGRs in non-IID settings: the curse of dimensionality and gradient heterogeneity. In order to address this issue, we propose GAS, a \shorten approach that can successfully adapt existing robust AGRs to non-IID settings. We also provide a detailed convergence analysis when the existing robust AGRs are combined with GAS. Experiments on various real-world datasets verify the efficacy of our proposed GAS. The implementation code is provided in https://github.com/YuchenLiu-a/byzantine-gas.

==> tabulars/cifar10.tex <==
\begin{tabular}{lcccccc}
\toprule
Attack & BitFlip & LabelFlip & LIE & Min-Max & Min-Sum & IPM \\
\midrule
Multi-Krum & 43.19 $\pm$ 0.38 & 43.90 $\pm$ 0.03 & 10.00 $\pm$ 0.00 & 10.00 $\pm$ 0.00 & 23.68 $\pm$ 0.18 & 10.00 $\pm$ 0.00 \\
Multi-Krum+\proposedmethod & \textbf{59.23} $\pm$ 0.55 & \textbf{61.47} $\pm$ 0.26 & \textbf{55.66} $\pm$ 0.93 & \textbf{49.19} $\pm$ 0.72 & \textbf{53.59} $\pm$ 0.96 & \textbf{56.94} $\pm$ 3.60 \\
\midrule
Bulyan & 54.10 $\pm$ 0.19 & 55.12 $\pm$ 0.14 & 30.58 $\pm$ 0.75 & 29.03 $\pm$ 1.10 & 46.19 $\pm$ 0.92 & 33.88 $\pm$ 0.61 \\
Bulyan+\proposedmethod & \textbf{59.14} $\pm$ 0.01 & \textbf{61.21} $\pm$ 0.60 & \textbf{48.90} $\pm$ 0.83 & \textbf{48.35} $\pm$ 1.58 & \textbf{53.74} $\pm$ 0.71 & \textbf{56.53} $\pm$ 1.51 \\
\midrule
Median & 45.41 $\pm$ 0.44 & 51.88 $\pm$ 0.62 & 28.75 $\pm$ 0.35 & 32.72 $\pm$ 0.81 & 37.39 $\pm$ 0.90 & 43.21 $\pm$ 0.47 \\
Median+\proposedmethod & \textbf{59.28} $\pm$ 0.24 & \textbf{61.24} $\pm$ 1.34 & \textbf{46.60} $\pm$ 0.13 & \textbf{49.37} $\pm$ 1.13 & \textbf{53.32} $\pm$ 1.90 & \textbf{56.33} $\pm$ 0.82 \\
\midrule
RFA & 49.61 $\pm$ 0.31 & 44.35 $\pm$ 0.31 & 15.39 $\pm$ 0.37 & 16.62 $\pm$ 0.83 & 18.22 $\pm$ 0.43 & 45.92 $\pm$ 0.13 \\
RFA+\proposedmethod & \textbf{53.35} $\pm$ 0.30 & \textbf{62.25} $\pm$ 0.56 & \textbf{52.69} $\pm$ 0.89 & \textbf{52.64} $\pm$ 1.48 & \textbf{56.16} $\pm$ 0.91 & \textbf{62.26} $\pm$ 1.27 \\
\midrule
DnC & 58.63 $\pm$ 1.29 & 60.82 $\pm$ 1.56 & 61.07 $\pm$ 0.72 & 60.42 $\pm$ 0.59 & 53.71 $\pm$ 0.96 & \textbf{59.99} $\pm$ 0.82 \\
DnC+\proposedmethod & \textbf{58.96} $\pm$ 0.60 & \textbf{61.02} $\pm$ 0.27 & \textbf{61.87} $\pm$ 0.51 & \textbf{61.04} $\pm$ 1.18 & \textbf{54.36} $\pm$ 1.12 & 57.92 $\pm$ 1.71 \\
\midrule
RBTM & 54.27 $\pm$ 1.63 & 59.60 $\pm$ 1.76 & 47.67 $\pm$ 2.51 & 49.02 $\pm$ 0.31 & 50.74 $\pm$ 0.06 & 55.27 $\pm$ 1.60 \\
RBTM+\proposedmethod & \textbf{59.41} $\pm$ 0.20 & \textbf{60.75} $\pm$ 0.19 & \textbf{52.10} $\pm$ 1.28 & \textbf{49.60} $\pm$ 0.17 & \textbf{53.63} $\pm$ 0.58 & \textbf{56.65} $\pm$ 1.52 \\
\bottomrule
\end{tabular}


==> tabulars/femnist.tex <==
\begin{tabular}{lcccccc}
\toprule
Attack & BitFlip & LabelFlip & LIE & Min-Max & Min-Sum & IPM \\
\midrule
Multi-Krum & 67.65 $\pm$ 0.23 & 57.43 $\pm$ 1.25 & 44.58 $\pm$ 0.07 & 28.32 $\pm$ 0.31 & 29.98 $\pm$ 0.45 & 12.26 $\pm$ 1.34 \\
Multi-Krum+\proposedmethod & \textbf{84.29} $\pm$ 1.76 & \textbf{85.45} $\pm$ 0.40 & \textbf{74.76} $\pm$ 1.74 & \textbf{57.46} $\pm$ 0.33 & \textbf{70.65} $\pm$ 1.35 & \textbf{81.46} $\pm$ 0.18 \\
\midrule
Bulyan & 77.58 $\pm$ 1.30 & 79.39 $\pm$ 2.14 & 56.43 $\pm$ 0.45 & 35.10 $\pm$ 0.69 & 44.83 $\pm$ 1.40 & 5.91 $\pm$ 0.17 \\
Bulyan+\proposedmethod & \textbf{84.90} $\pm$ 0.69 & \textbf{83.68} $\pm$ 0.76 & \textbf{71.43} $\pm$ 1.07 & \textbf{66.22} $\pm$ 0.47 & \textbf{71.76} $\pm$ 0.99 & \textbf{82.97} $\pm$ 1.04 \\
\midrule
Median & 80.25 $\pm$ 0.06 & 76.86 $\pm$ 1.96 & 64.88 $\pm$ 0.23 & 50.67 $\pm$ 0.37 & 61.33 $\pm$ 0.13 & 71.98 $\pm$ 0.77 \\
Median+\proposedmethod & \textbf{84.59} $\pm$ 0.14 & \textbf{85.67} $\pm$ 0.48 & \textbf{76.19} $\pm$ 0.43 & \textbf{65.84} $\pm$ 0.41 & \textbf{70.84} $\pm$ 0.86 & \textbf{82.18} $\pm$ 0.40 \\
\midrule
RFA & 5.46 $\pm$ 0.06 & 5.46 $\pm$ 0.01 & 5.46 $\pm$ 0.05 & 5.46 $\pm$ 0.03 & 5.46 $\pm$ 0.02 & 5.59 $\pm$ 0.09 \\
RFA+\proposedmethod & \textbf{84.86} $\pm$ 0.78 & \textbf{84.59} $\pm$ 0.20 & \textbf{69.82} $\pm$ 0.33 & \textbf{69.18} $\pm$ 0.09 & \textbf{77.67} $\pm$ 1.31 & \textbf{86.08} $\pm$ 2.51 \\
\midrule
DnC & 8.90 $\pm$ 0.31 & 5.59 $\pm$ 0.03 & 78.52 $\pm$ 0.28 & 5.46 $\pm$ 0.37 & 74.18 $\pm$ 0.03 & 74.70 $\pm$ 1.57 \\
DnC+\proposedmethod & \textbf{84.71} $\pm$ 0.39 & \textbf{85.39} $\pm$ 0.64 & \textbf{82.54} $\pm$ 0.26 & \textbf{74.37} $\pm$ 0.50 & \textbf{75.41} $\pm$ 0.22 & \textbf{82.73} $\pm$ 1.22 \\
\midrule
RBTM & 82.57 $\pm$ 0.34 & 81.57 $\pm$ 1.12 & 59.93 $\pm$ 0.20 & 65.20 $\pm$ 0.60 & 71.82 $\pm$ 0.73 & 76.88 $\pm$ 1.75 \\
RBTM+\proposedmethod & \textbf{84.89} $\pm$ 1.94 & \textbf{85.44} $\pm$ 0.20 & \textbf{73.38} $\pm$ 0.31 & \textbf{66.24} $\pm$ 0.94 & \textbf{75.50} $\pm$ 1.13 & \textbf{82.58} $\pm$ 1.85 \\
\bottomrule
\end{tabular}


==> tabulars/group_number.tex <==

\begin{tabular}{lcccccccc}
\toprule
Defense & \# Groups & Bit Flip & Label Flip & LIE & Min-Max & Min-Sum & IPM \\
\midrule
\multirow{2}{*}{\proposedmethod-Median} & 5 & 59.74 & 60.57 & 47.29 & 49.40 & 52.86 & 56.53 \\
& 100 & 59.74 & 60.97 & 46.12 & 50.69 & 53.36 & 56.84 \\
\midrule
\multirow{2}{*}{\proposedmethod-Trmean} & 5 & 59.20 & 61.05 & 48.72 & 49.62 & 53.06 & 56.58 \\
& 100 & 60.12 & 61.18 & 48.96 & 48.53 & 53.55 & 57.21 \\
\midrule
\multirow{2}{*}{\proposedmethod-Bulyan} & 5 & 59.45 & 60.40 & 50.18 & 49.48 & 53.33 & 56.45 \\
& 100 & 58.92 & 60.62 & 50.08 & 49.18 & 52.99 & 56.07 \\
\midrule
\multirow{2}{*}{\proposedmethod-Krum} & 5 & 59.89 & 61.91 & 54.42 & 50.55 & 53.11 & 56.63 \\
& 100 & 59.47 & 61.56 & 54.02 & 51.14 & 53.30 & 56.75 \\
\midrule
\multirow{2}{*}{\proposedmethod-RFA} & 5 & 55.92 & 61.52 & 53.00 & 53.58 & 55.07 & 61.79 \\
& 100 & 54.18 & 62.37 & 52.68 & 53.56 & 54.89 & 62.39 \\
\midrule
\multirow{2}{*}{\proposedmethod-DnC} & 5 & 58.09 & 60.75 & 62.10 & 59.75 & 53.73 & 58.35 \\
& 100 & 58.46 & 60.81 & 62.28 & 61.15 & 53.43 & 58.18 \\
\bottomrule
\end{tabular}

==> tabulars/imagenet12.tex <==
\begin{tabular}{lcccccc}
\toprule
Defense & BitFlip & LabelFlip & LIE & Min-Max & Min-Sum & IPM \\
\midrule
Multi-Krum & 44.36 $\pm$ 1.52 & 34.04 $\pm$ 1.69 & 45.38 $\pm$ 1.04 & 48.72 $\pm$ 0.16 & 57.69 $\pm$ 0.30 & 33.14 $\pm$ 0.86 \\
Multi-Krum+\proposedmethod & \textbf{66.79} $\pm$ 1.08 & \textbf{63.04} $\pm$ 0.14 & \textbf{57.15} $\pm$ 0.19 & \textbf{59.94} $\pm$ 0.32 & \textbf{64.07} $\pm$ 1.38 & \textbf{61.92} $\pm$ 0.04 \\
\midrule
Bulyan & 62.28 $\pm$ 0.84 & 59.84 $\pm$ 1.09 & 48.04 $\pm$ 2.22 & 48.97 $\pm$ 1.87 & 59.94 $\pm$ 0.51 & 60.67 $\pm$ 0.07 \\
Bulyan+\proposedmethod & \textbf{66.76} $\pm$ 0.72 & \textbf{62.28} $\pm$ 0.32 & \textbf{57.44} $\pm$ 0.39 & \textbf{58.81} $\pm$ 0.05 & \textbf{65.00} $\pm$ 0.08 & \textbf{62.76} $\pm$ 0.14 \\
\midrule
Median & 55.93 $\pm$ 0.55 & 58.14 $\pm$ 0.18 & 46.67 $\pm$ 1.01 & 49.07 $\pm$ 1.19 & 58.40 $\pm$ 0.03 & 43.62 $\pm$ 1.72 \\
Median+\proposedmethod & \textbf{66.28} $\pm$ 0.41 & \textbf{62.34} $\pm$ 1.10 & \textbf{60.74} $\pm$ 1.24 & \textbf{59.26} $\pm$ 0.31 & \textbf{64.78} $\pm$ 2.10 & \textbf{62.24} $\pm$ 0.51 \\
\midrule
RFA & 61.12 $\pm$ 1.26 & 61.31 $\pm$ 1.68 & 49.49 $\pm$ 1.33 & 53.04 $\pm$ 0.13 & 61.92 $\pm$ 0.67 & 63.97 $\pm$ 0.93 \\
RFA+\proposedmethod & \textbf{66.92} $\pm$ 1.58 & \textbf{63.88} $\pm$ 0.94 & \textbf{61.41} $\pm$ 0.02 & \textbf{59.42} $\pm$ 0.64 & \textbf{67.02} $\pm$ 0.54 & \textbf{66.67} $\pm$ 0.38 \\
\midrule
DnC & 54.94 $\pm$ 0.04 & 5.59 $\pm$ 0.06 & 58.01 $\pm$ 1.52 & 58.11 $\pm$ 0.41 & 60.42 $\pm$ 1.60 & 59.99 $\pm$ 0.50 \\
DnC+\proposedmethod & \textbf{65.19} $\pm$ 1.63 & \textbf{63.01} $\pm$ 0.27 & \textbf{64.42} $\pm$ 0.19 & \textbf{65.03} $\pm$ 1.23 & \textbf{65.38} $\pm$ 1.68 & \textbf{65.03} $\pm$ 0.04 \\
\midrule
RBTM & 60.06 $\pm$ 1.76 & 60.44 $\pm$ 0.37 & 55.77 $\pm$ 0.82 & 57.50 $\pm$ 0.10 & 63.91 $\pm$ 0.78 & 56.19 $\pm$ 1.05 \\
RBTM+\proposedmethod & \textbf{66.99} $\pm$ 0.38 & \textbf{61.92} $\pm$ 1.22 & \textbf{59.87} $\pm$ 0.72 & \textbf{59.81} $\pm$ 1.34 & \textbf{64.94} $\pm$ 0.72 & \textbf{63.40} $\pm$ 0.97 \\
\bottomrule
\end{tabular}


==> tabulars/main_experiments_2x2.tex <==

\begin{tabular}{l|cccccc|cccccc}
\toprule
Dataset & \multicolumn{6}{c|}{CIFAR-10} & \multicolumn{6}{c}{CIFAR-100}\\
\midrule
Attack & BitFlip & LabelFlip & LIE & Min-Max & Min-Sum & IPM & BitFlip & LabelFlip & LIE & Min-Max & Min-Sum & IPM \\
\midrule
Multi-Krum & 43.19 $\pm$ 0.38 & 43.90 $\pm$ 0.03 & 37.03 $\pm$ 1.62 & 39.06 $\pm$ 0.07 & 23.68 $\pm$ 0.18 & 36.47 $\pm$ 0.22 & 34.27 $\pm$ 0.28 & 35.57 $\pm$ 0.94 & 17.17 $\pm$ 0.08 & 16.77 $\pm$ 0.78 & 22.89 $\pm$ 0.61 & 15.93 $\pm$ 2.00 \\
Multi-Krum+\proposedmethod & \textbf{59.23} $\pm$ 0.55 & \textbf{61.47} $\pm$ 0.26 & \textbf{55.66} $\pm$ 0.93 & \textbf{49.19} $\pm$ 0.72 & \textbf{53.59} $\pm$ 0.96 & \textbf{56.94} $\pm$ 3.60 & \textbf{42.41} $\pm$ 0.58 & \textbf{42.55} $\pm$ 0.12 & \textbf{27.81} $\pm$ 0.32 & \textbf{31.18} $\pm$ 1.48 & \textbf{41.33} $\pm$ 0.50 & \textbf{42.62} $\pm$ 1.53 \\
\midrule
Bulyan & 54.10 $\pm$ 0.19 & 55.12 $\pm$ 0.14 & 30.58 $\pm$ 0.75 & 29.03 $\pm$ 1.10 & 46.19 $\pm$ 0.92 & 33.88 $\pm$ 0.61 & 35.77 $\pm$ 0.18 & 42.60 $\pm$ 0.07 & 35.41 $\pm$ 0.40 & 35.53 $\pm$ 1.38 & 39.13 $\pm$ 0.12 & 40.27 $\pm$ 1.64 \\
Bulyan+\proposedmethod & \textbf{59.14} $\pm$ 0.01 & \textbf{61.21} $\pm$ 0.60 & \textbf{48.90} $\pm$ 0.83 & \textbf{48.35} $\pm$ 1.58 & \textbf{53.74} $\pm$ 0.71 & \textbf{56.53} $\pm$ 1.51 & \textbf{42.28} $\pm$ 1.61 & \textbf{43.77} $\pm$ 0.46 & \textbf{38.39} $\pm$ 0.19 & \textbf{36.33} $\pm$ 1.51 & \textbf{40.73} $\pm$ 0.39 & \textbf{42.88} $\pm$ 0.14 \\
\midrule
Median & 45.41 $\pm$ 0.44 & 51.88 $\pm$ 0.62 & 28.75 $\pm$ 0.35 & 32.72 $\pm$ 0.81 & 37.39 $\pm$ 0.90 & 43.21 $\pm$ 0.47 & 36.62 $\pm$ 0.12 & 41.64 $\pm$ 0.76 & 22.75 $\pm$ 0.04 & 23.21 $\pm$ 0.71 & 30.68 $\pm$ 0.26 & 40.98 $\pm$ 0.38 \\
Median+\proposedmethod & \textbf{59.28} $\pm$ 0.24 & \textbf{61.24} $\pm$ 1.34 & \textbf{46.60} $\pm$ 0.13 & \textbf{49.37} $\pm$ 1.13 & \textbf{53.32} $\pm$ 1.90 & \textbf{56.33} $\pm$ 0.82 & \textbf{42.41} $\pm$ 0.66 & \textbf{42.62} $\pm$ 0.09 & \textbf{35.16} $\pm$ 1.08 & \textbf{36.46} $\pm$ 0.10 & \textbf{41.08} $\pm$ 0.04 & \textbf{43.63} $\pm$ 2.85 \\
\midrule
RFA & 49.61 $\pm$ 0.31 & 44.35 $\pm$ 0.31 & 15.39 $\pm$ 0.37 & 16.62 $\pm$ 0.83 & 18.22 $\pm$ 0.43 & 45.92 $\pm$ 0.13 & 21.32 $\pm$ 0.84 & 28.76 $\pm$ 1.33 & 25.63 $\pm$ 0.20 & 26.46 $\pm$ 1.83 & 28.33 $\pm$ 0.93 & 21.36 $\pm$ 0.54 \\
RFA+\proposedmethod & \textbf{53.35} $\pm$ 0.30 & \textbf{62.25} $\pm$ 0.56 & \textbf{52.69} $\pm$ 0.89 & \textbf{52.64} $\pm$ 1.48 & \textbf{56.16} $\pm$ 0.91 & \textbf{62.26} $\pm$ 1.27 & \textbf{42.64} $\pm$ 0.44 & \textbf{42.42} $\pm$ 0.25 & \textbf{26.30} $\pm$ 1.08 & \textbf{30.30} $\pm$ 0.12 & \textbf{41.09} $\pm$ 0.66 & \textbf{43.45} $\pm$ 0.52 \\
\midrule
DnC & 58.63 $\pm$ 1.29 & 60.82 $\pm$ 1.56 & 61.07 $\pm$ 0.72 & 60.42 $\pm$ 0.59 & 53.71 $\pm$ 0.96 & \textbf{59.99} $\pm$ 0.82 & 41.77 $\pm$ 0.62 & 42.93 $\pm$ 0.07 & 42.95 $\pm$ 1.03 & 40.15 $\pm$ 0.70 & 40.02 $\pm$ 1.07 & 41.23 $\pm$ 2.29 \\
DnC+\proposedmethod & \textbf{58.96} $\pm$ 0.60 & \textbf{61.02} $\pm$ 0.27 & \textbf{61.87} $\pm$ 0.51 & \textbf{61.04} $\pm$ 1.18 & \textbf{54.36} $\pm$ 1.12 & 57.92 $\pm$ 1.71 & \textbf{43.35} $\pm$ 0.41 & \textbf{43.57} $\pm$ 1.11 & \textbf{43.64} $\pm$ 0.11 & \textbf{41.66} $\pm$ 0.78 & \textbf{41.02} $\pm$ 1.39 & \textbf{43.25} $\pm$ 0.43 \\
\midrule
RBTM & 54.27 $\pm$ 1.63 & 59.60 $\pm$ 1.76 & 47.67 $\pm$ 2.51 & 49.02 $\pm$ 0.31 & 50.74 $\pm$ 0.06 & 55.27 $\pm$ 1.60 & 36.35 $\pm$ 0.17 & 42.67 $\pm$ 1.55 & 24.06 $\pm$ 0.09 & 26.24 $\pm$ 1.04 & 36.51 $\pm$ 0.40 & 43.12 $\pm$ 1.12 \\
RBTM+\proposedmethod & \textbf{59.41} $\pm$ 0.20 & \textbf{60.75} $\pm$ 0.19 & \textbf{52.10} $\pm$ 1.28 & \textbf{49.60} $\pm$ 0.17 & \textbf{53.63} $\pm$ 0.58 & \textbf{56.65} $\pm$ 1.52 & \textbf{43.44} $\pm$ 0.81 & \textbf{43.19} $\pm$ 2.65 & \textbf{33.14} $\pm$ 0.58 & \textbf{34.35} $\pm$ 0.76 & \textbf{41.51} $\pm$ 0.93 & \textbf{43.20} $\pm$ 0.76 \\
\midrule
Dataset & \multicolumn{6}{c|}{FEMNIST} & \multicolumn{6}{c}{ImageNet-12}\\
\midrule
Attack & BitFlip & LabelFlip & LIE & Min-Max & Min-Sum & IPM & BitFlip & LabelFlip & LIE & Min-Max & Min-Sum & IPM \\
\midrule
Multi-Krum & 67.65 $\pm$ 0.23 & 57.43 $\pm$ 1.25 & 44.58 $\pm$ 0.07 & 28.32 $\pm$ 0.31 & 29.98 $\pm$ 0.45 & 12.26 $\pm$ 1.34 & 44.36 $\pm$ 1.52 & 34.04 $\pm$ 1.69 & 45.38 $\pm$ 1.04 & 48.72 $\pm$ 0.16 & 57.69 $\pm$ 0.30 & 33.14 $\pm$ 0.86 \\
Multi-Krum+\proposedmethod & \textbf{84.29} $\pm$ 1.76 & \textbf{85.45} $\pm$ 0.40 & \textbf{74.76} $\pm$ 1.74 & \textbf{57.46} $\pm$ 0.33 & \textbf{70.65} $\pm$ 1.35 & \textbf{81.46} $\pm$ 0.18 & \textbf{66.79} $\pm$ 1.08 & \textbf{63.04} $\pm$ 0.14 & \textbf{57.15} $\pm$ 0.19 & \textbf{59.94} $\pm$ 0.32 & \textbf{64.07} $\pm$ 1.38 & \textbf{61.92} $\pm$ 0.04 \\
\midrule
Bulyan & 77.58 $\pm$ 1.30 & 79.39 $\pm$ 2.14 & 56.43 $\pm$ 0.45 & 35.10 $\pm$ 0.69 & 44.83 $\pm$ 1.40 & 5.91 $\pm$ 0.17 & 62.28 $\pm$ 0.84 & 59.84 $\pm$ 1.09 & 48.04 $\pm$ 2.22 & 48.97 $\pm$ 1.87 & 59.94 $\pm$ 0.51 & 60.67 $\pm$ 0.07 \\
Bulyan+\proposedmethod & \textbf{84.90} $\pm$ 0.69 & \textbf{83.68} $\pm$ 0.76 & \textbf{71.43} $\pm$ 1.07 & \textbf{66.22} $\pm$ 0.47 & \textbf{71.76} $\pm$ 0.99 & \textbf{82.97} $\pm$ 1.04 & \textbf{66.76} $\pm$ 0.72 & \textbf{62.28} $\pm$ 0.32 & \textbf{57.44} $\pm$ 0.39 & \textbf{58.81} $\pm$ 0.05 & \textbf{65.00} $\pm$ 0.08 & \textbf{62.76} $\pm$ 0.14 \\
\midrule
Median & 80.25 $\pm$ 0.06 & 76.86 $\pm$ 1.96 & 64.88 $\pm$ 0.23 & 50.67 $\pm$ 0.37 & 61.33 $\pm$ 0.13 & 71.98 $\pm$ 0.77 & 55.93 $\pm$ 0.55 & 58.14 $\pm$ 0.18 & 46.67 $\pm$ 1.01 & 49.07 $\pm$ 1.19 & 58.40 $\pm$ 0.03 & 43.62 $\pm$ 1.72 \\
Median+\proposedmethod & \textbf{84.59} $\pm$ 0.14 & \textbf{85.67} $\pm$ 0.48 & \textbf{76.19} $\pm$ 0.43 & \textbf{65.84} $\pm$ 0.41 & \textbf{70.84} $\pm$ 0.86 & \textbf{82.18} $\pm$ 0.40 & \textbf{66.28} $\pm$ 0.41 & \textbf{62.34} $\pm$ 1.10 & \textbf{60.74} $\pm$ 1.24 & \textbf{59.26} $\pm$ 0.31 & \textbf{64.78} $\pm$ 2.10 & \textbf{62.24} $\pm$ 0.51 \\
\midrule
RFA & 5.46 $\pm$ 0.06 & 5.46 $\pm$ 0.01 & 5.46 $\pm$ 0.05 & 5.46 $\pm$ 0.03 & 5.46 $\pm$ 0.02 & 5.59 $\pm$ 0.09 & 61.12 $\pm$ 1.26 & 61.31 $\pm$ 1.68 & 49.49 $\pm$ 1.33 & 53.04 $\pm$ 0.13 & 61.92 $\pm$ 0.67 & 63.97 $\pm$ 0.93 \\
RFA+\proposedmethod & \textbf{84.86} $\pm$ 0.78 & \textbf{84.59} $\pm$ 0.20 & \textbf{69.82} $\pm$ 0.33 & \textbf{69.18} $\pm$ 0.09 & \textbf{77.67} $\pm$ 1.31 & \textbf{86.08} $\pm$ 2.51 & \textbf{66.92} $\pm$ 1.58 & \textbf{63.88} $\pm$ 0.94 & \textbf{61.41} $\pm$ 0.02 & \textbf{59.42} $\pm$ 0.64 & \textbf{67.02} $\pm$ 0.54 & \textbf{66.67} $\pm$ 0.38 \\
\midrule
DnC & 8.90 $\pm$ 0.31 & 77.71 $\pm$ 0.03 & 78.52 $\pm$ 0.28 & 8.29 $\pm$ 0.37 & 74.18 $\pm$ 0.03 & 74.70 $\pm$ 1.57 & 54.94 $\pm$ 0.04 & 5.59 $\pm$ 0.06 & 58.01 $\pm$ 1.52 & 58.11 $\pm$ 0.41 & 60.42 $\pm$ 1.60 & 59.99 $\pm$ 0.50 \\
DnC+\proposedmethod & \textbf{84.71} $\pm$ 0.39 & \textbf{85.39} $\pm$ 0.64 & \textbf{82.54} $\pm$ 0.26 & \textbf{74.37} $\pm$ 0.50 & \textbf{75.41} $\pm$ 0.22 & \textbf{82.73} $\pm$ 1.22 & \textbf{65.19} $\pm$ 1.63 & \textbf{63.01} $\pm$ 0.27 & \textbf{64.42} $\pm$ 0.19 & \textbf{65.03} $\pm$ 1.23 & \textbf{65.38} $\pm$ 1.68 & \textbf{65.03} $\pm$ 0.04 \\
\midrule
RBTM & 82.57 $\pm$ 0.34 & 81.57 $\pm$ 1.12 & 59.93 $\pm$ 0.20 & 65.20 $\pm$ 0.60 & 71.82 $\pm$ 0.73 & 76.88 $\pm$ 1.75 & 60.06 $\pm$ 1.76 & 60.44 $\pm$ 0.37 & 55.77 $\pm$ 0.82 & 57.50 $\pm$ 0.10 & 63.91 $\pm$ 0.78 & 56.19 $\pm$ 1.05 \\
RBTM+\proposedmethod & \textbf{84.89} $\pm$ 1.94 & \textbf{85.44} $\pm$ 0.20 & \textbf{73.38} $\pm$ 0.31 & \textbf{66.24} $\pm$ 0.94 & \textbf{75.50} $\pm$ 1.13 & \textbf{82.58} $\pm$ 1.85 & \textbf{66.99} $\pm$ 0.38 & \textbf{61.92} $\pm$ 1.22 & \textbf{59.87} $\pm$ 0.72 & \textbf{59.81} $\pm$ 1.34 & \textbf{64.94} $\pm$ 0.72 & \textbf{63.40} $\pm$ 0.97 \\
\bottomrule
\end{tabular}
